MemFold: Learning Compact Soft Memory for Long-Context Personalization via On-Policy Optimization

An assistant that serves the same user over a long horizon has to answer from what that user has revealed: which preferences still hold, which were revised, and which constraints apply now. Retaining that information is not the same as acting on it, and the two are usually optimized as if they were. Keeping the information as text makes the reader's input grow with the retained history, while compressing it into a fixed number of latent vectors bounds the interface but is typically trained to reconstruct text or imitate reference answers, both of which are scored on sequences the reader never produced. We present MemFold, which optimizes a fixed-budget soft memory by the behavior it supports. A query-conditioned textual memory is compressed into K continuous vectors that form the reader's memory interface, and the reader is then trained on its own rollouts under two complementary signals: group-relative rewards for task outcomes, and confidence-gated on-policy distillation in which a frozen textual-memory teacher re-scores the student's sampled tokens under the textual memory. The teacher is never sampled from, so supervision stays on the student's current distribution and adds no autoregressive decoding; at inference it is removed entirely. Across three Qwen backbones, MemFold attains the highest accuracy we measure on PersonaMem-32K and PersonaMem-128K, with margins that widen at the longer history length, and transfers to PrefEval and LongMemEval without target-domain training. Ablations attribute most of the task gain to the reward term and a smaller additional gain to the teacher signal, and memory interventions show that the reader depends on the instance-specific content of its soft memory.

==> packages.tex <==
%% packages.tex —— 全部 LaTeX 包的统一入口
%% 由 MITcsail.cls 在 \LoadClass 之后 \input 进来
%% 顺序：math → 排版/字体 → 颜色 → 图 → caption → 表格 → 布局 → 工具 → 算法 → bib → hyperref（最后）

%%==================== Math ====================
\RequirePackage{amsmath}                  % AMS 数学环境基础（align / equation 等）
\RequirePackage{amsthm}                   % 定理 / 引理 / 证明等环境
\RequirePackage{amssymb}                  % AMS 数学符号扩展（含 \mathbb 等，自动覆盖 amsfonts）
\RequirePackage{mathtools}                % amsmath 增强（\DeclarePairedDelimiter 等），必须在 amsmath 之后
\RequirePackage{bm}                       % 粗体数学符号 \bm{...}（math_commands.tex 中 \vzero 等依赖）
\RequirePackage{mathpazo}                 % Palatino 风格数学字体

%%==================== 排版 / 字体 ====================
\RequirePackage{microtype}                % 微排版（字距、保护性紧排、整体字面更整齐）
\RequirePackage{anyfontsize}              % 解除字号必须匹配 metric 的限制（\fontsize 任意值）
\RequirePackage{titlesec}                 % 章节标题样式控制（\titlelabel 用到）
\RequirePackage{tocloft}                  % ToC 样式控制（section / subsection 行距）
\RequirePackage[defaultsans]{lato}         % 无衬线 Lato → \sfdefault；正文仍 Palatino（rmdefault 不变）
\RequirePackage{iftex}                     % 按编译引擎选择标题字体实现
\ifPDFTeX
  \newcommand{\AvenirTitleFamily}{\sffamily}
  \PackageWarningNoLine{arxivtmpl}{Avenir requires XeLaTeX or LuaLaTeX; falling back to sans-serif for the title}
\else
  \RequirePackage[no-math]{fontspec}
  \newfontfamily\AvenirTitleFamily[
    Path=fonts/,
    UprightFont=AvenirLT-Regular.ttf,
    BoldFont=AvenirLT-Bold.ttf,
    ItalicFont=AvenirLT-Oblique.ttf,
    BoldItalicFont=AvenirLT-BoldOblique.ttf
  ]{Avenir}
\fi

%%==================== 颜色 ====================
\RequirePackage[table,dvipsnames]{xcolor}       % 颜色（\definecolor / \textcolor / \fcolorbox + MidnightBlue / NavyBlue / Maroon 等命名色）
\RequirePackage{colortbl}                 % 表格行/列/单元颜色（\rowcolor 等）

%%==================== 图与排版插入 ====================
\RequirePackage{graphicx}                 % \includegraphics
\RequirePackage{wrapfig}                  % 文字环绕图（\begin{wrapfigure}）
\RequirePackage{adjustbox}                % \adjustbox 缩放 / 裁剪 / 对齐
\RequirePackage{tikz}                     % TikZ 绘图（\circled 命令依赖）

%%==================== Caption ====================
\RequirePackage[labelsep=colon]{caption}  % caption 标签样式（"Figure 1: ..."）
\RequirePackage{subcaption}               % sub-figure / sub-table caption，必须在 caption 之后

%%==================== 表格 ====================
\RequirePackage{booktabs}                 % 三线表（\toprule / \midrule / \bottomrule）
\RequirePackage{multirow}                 % 表格跨行（\multirow{...}）
\RequirePackage{tabularx}                 % 自适应列宽表格
\RequirePackage{makecell}                 % 单元格内换行（\makecell）

%%==================== 布局 ====================
\RequirePackage{geometry}                 % 页面四周边距（在 cls 中 \geometry{...} 设置，对齐 MAI 报告）
\RequirePackage{fancyhdr}                 % 自定义 header / footer
\RequirePackage{authblk}                  % 多作者 / 多 affiliation
\RequirePackage{enumitem}                 % list 自定义（itemsep / topsep / label 等）
\RequirePackage[most]{tcolorbox}                % 彩色 box / 提示框

%%==================== 工具 ====================
\RequirePackage{datetime}                 % 日期格式（\newdateformat{ymd}{...} 用于页眉）
\RequirePackage{verbatim}                 % verbatim 输出 / \begin{comment}
\RequirePackage{pifont}                   % \cmark / \xmark 等 dingbats 符号

% Algorithm packages are shared with the manuscript in paper_preamble.tex.

%%==================== Bib ====================
\RequirePackage[numbers,sort&compress]{natbib}            % 数字引用 [1,2,3]，自动排序与合并

%%==================== Hyperref（必须最后加载）====================
%% ---- Google-brand palette (single source; see CLAUDE.md "Color palette") ----
%% 全局唯一非黑色来源，取自 writing/skills/plot/style.py（brand 档）。
%% 新增非黑色只能用这组或其 xcolor 混白浓度（如 gblue!22），不要再 \definecolor 新色。
\definecolor{gblue}{HTML}{4285F4}
\definecolor{gred}{HTML}{DB4437}
\definecolor{gyellow}{HTML}{F4B400}
\definecolor{ggreen}{HTML}{0F9D58}
\definecolor{gpurple}{HTML}{AB47BC}
\definecolor{ggrey}{HTML}{5F6368}
\colorlet{linkcol}{gblue}                                        % = palette blue，所有超链接统一色
\RequirePackage[colorlinks=true,allcolors=linkcol]{hyperref}               % 彩色文字链接（无边框/下划线）
\RequirePackage[capitalize,noabbrev]{cleveref}                              % \Cref / \cref（必须在 hyperref 之后）
%% 显式强制蓝灰文字链接、无边框（防止其它包/默认值覆盖）
\hypersetup{colorlinks=true,linkcolor=linkcol,citecolor=linkcol,urlcolor=linkcol,pdfborder={0 0 0}}

